Understanding Video Transformers via Universal Concept Discovery

This paper studies the problem of concept-based interpretability of transformer representations for videos. Concretely, we seek to explain the decision-making process of video transformers based on high-level, spatiotemporal concepts that are automatically discovered. Prior research on concept-based interpretability has concentrated solely on image-level tasks. Comparatively, video models deal with the added temporal dimension, increasing complexity and posing challenges in identifying dynamic concepts over time. In this work, we systematically address these challenges by introducing the first Video Transformer Concept Discovery (VTCD) algorithm. To this end, we propose an efficient approach for unsupervised identification of units of video transformer representations - concepts, and ranking their importance to the output of a model. The resulting concepts are highly interpretable, revealing spatio-temporal reasoning mechanisms and object-centric representations in unstructured video models. Performing this analysis jointly over a diverse set of supervised and self-supervised representations, we discover that some of these mechanism are universal in video transformers. Finally, we show that VTCD can be used for fine-grained action recognition and video object segmentation.

==> sec/3_method_copy.tex <==
\section{Video transformer concept discovery}

% \begin{enumerate}
%     \item intro, definitions and goals
%     \item concept discovery
%     \begin{enumerate}
%         \item tubelet proposals
%         \item Concept Clustering via Convex Non-Negative Matrix Factorization
%     \end{enumerate}
%     \item Concept importance
%     \begin{enumerate}
%         \item Concept importance ranking
%         \item Concept Fidelity via CNMF weighting
%     \end{enumerate}
% \end{enumerate}

\subsection{Preliminaries}
We study the problem of decomposing a video transformer representation into a set of high-level concepts and ranking their importance for the model's predictions. Given a set of videos, $\textbf{x} \in \mathbb{R}^{N \times 3 \times T \times H \times W}$, and a model $f$, let $f_l$ denote the model layers up to layer $l$ and $f_l(\textbf{x}) = \textbf{z} \in \mathbb{R}^{N \times C \times T' \times H' \times W'}$ the intermediate representation of the model. 

To decompose $f_l(\textbf{x})$ into a set of human-interpretable concepts, $\textbf{C} = \{c_1, ..., c_i\}$, existing, image-level approaches~\cite{ghorbani2019towards, fel2023craft} first split the feature map into a set of $M$ proposal $\textbf{T} \in \mathbb{R}^{C \times M}$, where each $T_m$ corresponds to a region of the feature map. These proposal are then clustered into $Q << M$ concepts in the feature space of the model to form a cluster assignment matrix $W \in \mathbb{R}^{M \times Q}$. Finally, each concept $c_i$ is assigned an importance score $s_i$, that quantifies its importance to the model's prediction for a given task. Performing this analysis over all the layers in $f$ allows one to obtain a number of insights about the key units of the representation and their role in the decision process.

However, existing approaches are not immediately applicable to video transformers due to their insufficient scalability and over-reliance on 2D CNNs design. 
%inefficient proposal techniques, assumption of positive matrices, and frailty of importance scores. 
In this work, we extend concept-based interpetability to video representations. To this end, we first describe a novel proposal generation technique in Section~\ref{sec:Tublets} that operates over space-time feature volumes and outputs spatio-temporal regions (tublets). Next, in Section~\ref{sec:ConceptClustering} we adapt existing concept clustering technique to video transformer representations. In Section~\ref{sec:Importance} we propose CRIS - a novel concept importance estimation approach for transformer heads. Finally, inspired by previous work~\cite{dravid2023rosetta}, Section~\ref{sec:Rosetta} describe our method of finding \textit{Rosetta Concepts}, universal spatiotemporal concepts across multiple architectures and tasks.


\begin{figure*}
    \centering   
\includegraphics[width=\textwidth]{figures/methods/MainMethod1.pdf}
    \caption{Caption}
    \label{fig:MainMethod}
\end{figure*}

\subsection{Concept discovery}

\subsubsection{Tubelet proposals}\label{sec:Tublets}
% One may be tempted to perform supervised concept analysis, like done in TCAV~\cite{kim2018interpretability}, however it is not clear what concepts should be investigated apriori in spatiotemporal models (we show examples of strange concepts in Sec.~\ref{sec:Experiments}). Therefore, we choose to perform concept \textit{discovery}, where no labelled data or apriori sets of concepts are required.
% ICE~\cite{zhang2021invertible} directly cluster flattened features across the dataset without proposing segments, but video transformer architectures retain such high resolution features that clustering across a dataset of video features is not computationally feasible. 
% Concept discovery methods~\cite{dave2019towards, fel2023craft} have solely been applied to images until now and the techniques do not scale when naively applied to videos. ACE~\cite{ghorbani2019towards} proposes segments using RGB superpixels and CRAFT~\cite{fel2023craft} uses random crops of images as the segment proposals, however, the number of meaningful superpixels or crops in RGB space is exponentially greater for videos and it also is not constrained to capture any semantics in model feature space. 

Previous methods~\cite{ghorbani2019towards,fel2023craft,fel2023holistic} use superpixels or crops in RGB space to propose segments, however, the number of possible segments is exponentially greater for videos and these methods also are not constrained to capture any semantics in model feature space. We solve these issues by constructing tubelets in each video via Simple Linear Iterative Clustering~\cite{achanta2012slic,Ilic2020WACV} (SLIC) on the spatiotemporal features via
\begin{equation}
    \textbf{T} = \text{GAP}(\textbf{B} \odot \textbf{z}) = \text{GAP}(\text{SLIC}(\textbf{z}) \odot \textbf{z}) ,
\end{equation}
where $\textbf{T} \in \mathbb{R}^{C \times M} $ is the set of tubelets for the dataset, $\textbf{B} \in \{0,1\}^{C \times M \times N  \times T' \times H' \times W'}$ are the binary support masks obtained from the SLIC clustering, $M$ is the total number of tubelets for all $N$ videos ($M>>N$), and GAP is a global average pooling operation over space and time dimensions. 

SLIC is an extension of the K-Means algorithm that constrains cluster support masks to be connected. It has two main advantages, that are especially important in the video domain: (i) non-disjoint tubelets are easier to interpret for humans because they reduce the need to attend to multiple regions in a video at a time, and (ii) SLIC is robust to the number clusters hyperparameter as it automatically prunes spurious, disconnected tubelets. Next, we describe our approach for grouping individual tubeletes into higher-level concept clusters.
%one can overcluster with a larger number of tubelets and then let the connectivity step in SLIC prune spurious tubelets (\ie rather than rely on another hyperparameter, such as an elbow value or a hard set number of clusters). 
% \textcolor{red}{Visualizations of the tubelets generated via SLIC are shown in Fig.~\ref{}}
% Moreover, we demonstrate that SLIC admits faithful concepts compared with other methods (\eg Kmeans).

\subsubsection{Concept clustering}\label{sec:ConceptClustering}
% Given the dataset of semantically meaningful tubelets $\textbf{T}$, we perform clustering on the dataset to produce a set of concepts (\ie cluster centroids), where each concept is associated with a subset of the tubelets.
The initial work in concept discovery uses K-Means to cluster proposals into concepts~\cite{ghorbani2019towards}. More recently, several works~\cite{ding2008convex,zhang2021invertible, fel2023craft, fel2023holistic} have shown that Non-Negative Matrix Factorization (NMF) has beneficial properties compared to other dimensionality reduction or clustering techniques (\eg K-Means, PCA), such as a better trade off between the interpretability of discovered concepts and faithfulness to the model's representations. 
Given a non-negative data matrix, $\textbf{T} \in \mathbb{R}^{M \times C}$, NMF aims to find two non-negative matrices, $\textbf{W} \in \mathbb{R}^{M \times Q}$ and $\textbf{C} \in \mathbb{R}^{Q \times C}$, such that $\textbf{T} = \textbf{W} \textbf{C}$, where $\textbf{W}$ is the cluster assignment matrix. Unfortunately, NMF cannot be applied to transformer-based architectures as transformers generally do not use ReLU activation functions and contain negative values throughout the model. 

We solve this problem by leveraging Convex Non-negative Matrix Factorization~\cite{ding2008convex} (CNMF). CNMF is an extension of NMF where the factorization is constrained such that the columns of $\textbf{W}$ are convex combinations of the columns of $\textbf{T}$ (\ie each column of $\textbf{W}$ is a weighted average of the columns of $\textbf{T}$. This constraint can be written as
\begin{equation}
    \textbf{W} = \textbf{T} \textbf{G},
\end{equation}
where $\textbf{G} \in [0,1]^{C \times Q}$ and $\sum_j \textbf{G}_{i,j}=1$. To cluster a set of tublets, $\textbf{T}$, into corresponding concepts, we solve the equation
\begin{equation}
    (\textbf{G},\textbf{C}) = \argmin_{\textbf{C}>0,\textbf{G}>0} || \textbf{T} - \textbf{T} \textbf{G} \textbf{C} ||^2,
\end{equation}
where the final set of concepts are represented by the rows of the matrix $\textbf{C}$, \ie concept centroid $c_i$ is the $i^{th}$ row of $\textbf{C}$. We denote the full set of concepts as $\textbf{C}=\{c_1,...,c_i\}$.



% Given a dataset of spatiotemporally averaged tubelets, $\textbf{T}_l$, CNMF factorizes the input data via
% % \begin{equation}
%     % \textbf{T}_l = \textbf{T}_l \textbf{W} \textbf{G}^T,
% % \end{equation}
% \begin{equation}
%     (\textbf{W},\textbf{G}) = \argmin_{\textbf{W}>0,\textbf{G}>0} || \textbf{T}_l - \textbf{T}_l \textbf{W} \textbf{G}^T ||^2
% \end{equation}
% where $\textbf{G} \in [0,1]^{m \times q}$ is the (soft) cluster assignment matrix ($\sum_i G_{i,j}=1$) and $\textbf{W} \in \mathbb{R}^{m \times q}$ is a linear matrix that computes $q$ concept centroids. 


% CNMF has several useful properties beyond traditional NMF. First, it allows for negative values in the data matrix, making it applicable to any neural architecture representation. Second, for reasons of interpretability, it is designed such that the vectors defining the set of cluster centroids, $\{\textbf{C}\} = \{\textbf{C}_1^1, \textbf{C}_1^2, ..., \textbf{C}_2^1,\textbf{C}_2^2, ..., \textbf{C}_l^i \}$, lie within the column space of the data matrix, $\textbf{T}_l$, \ie for the single concept, $\textbf{C}^i$,
% \begin{equation}
    % \textbf{C}_l^i = (\textbf{T}_l \textbf{W}) = w_1^i \textbf{T}_{l_1} + w_2^i \textbf{T}_{l_2} + ... + w_m^i \textbf{T}_{l_m}.
% \end{equation}
% Thus, concepts are precisely composed of convex combinations of the tubelets and the assignment can be viewed explicitly via the matrix, $\textbf{G}$. Unlike KMeans, $\textbf{G}$ softley assigns each data point to a centroid, encouraging concepts to be compositional and interpretable~\cite{ding2008convex,zhang2021invertible,fel2023craft,fel2023holistic}. We use $\textbf{B}_l^{\textbf{C}^i}$ to denote the binary support masks that are obtained by considering the most closely assigned tubelets to concept $\textbf{C}_l^i$, \ie obtained through taking $\argmax_q (\textbf{G})$.

\subsection{Concept importance}\label{sec:Importance}
Given a set of discovered concepts in a video transformer, we now aim to quantify their impact on model performance.
% Moreover, recent work compared several concept importance methods~\cite{fel2023holistic} and showed that occlusion-based methods, \ie methods that recursively set concepts to a baseline value and calculate the performance drop, are provably optimal for the last layer of a classifier and achieve comparable performance to gradient based-methods (we demonstrate this empirically in Sec.~\ref{}). % do we need this line?
A necessary unit of study in transformers are the \textit{self-attention layers} (\ie queries, keys, values). Similar to findings in NLP literature~\cite{michel2019sixteen}, in Section~\ref{sec:ExpValidation} we demonstrate that recent concept importance methods applied to image models (\eg gradient-based~\cite{kim2018interpretability, ghorbani2019towards}, occlusion-based~\cite{fel2023holistic}) cannot accurately rank the importance of concepts contained in the self-attention layers due to the inherent robustness of transformers to small changes in these single units, \eg, manipulation a single attention head has no statistically significant impact on performance.

 % Several methods have been developed to quantify concept importance and have been successfully applied to CNN-based object recognition models (\eg gradient based methods~\cite{kim2018interpretability, fel2023holistic}, occlusion-based methods~\cite{fel2023holistic}).

Towards a solution to this problem, we propose \textbf{C}oncept \textbf{R}andomized \textbf{I}mportance \textbf{S}ampling (\ConceptRankAlgName), a general method to compute importance for any unit of interest (even beyond concepts, \eg we rank both concept and head importance in Sections~\ref{sec:Experiments} and~\ref{sec:Application}, respectively). CRIS is designed to account for the significant noise when occluding single concepts (visually presented in Fig.~\ref{fig:CRIS_Method}). 
%The key of \ConceptRankAlgName is to create a `global concept occlusion mask'; a mask that randomly occludes many concepts at a time across all layers (and heads) to ensure a performance decrease. This random sampling of global concept masking is repeated N times. Then the importance of a concept is calculated by the weighted average of the masks where the weights are the model performances. 
Formally, let $f_l$ denote the model up to layer $l$ and let $f'_l$ denote the model layers after layer $l$ (including the output layer). We construct global concept masks, $\textbf{M} = \{M_1, M_2, ..., M_{k}\} \in \mathcal{U} \{0,1\}^{Q}$, by randomly sampling a fraction ($\lambda$=0.5 in our experiments) of the $Q$ concepts to zero out at inference. Given a video, $\textbf{x}$, we pass it through the model while setting to zero all tokens belonging to concepts masked by $M_i$, as

\begin{equation}
    \hat y_i = f'_l( f_l(\textbf{x}) \odot B_i ),
\end{equation}
where $B_i \in \textbf{B}$ denotes the binary masks belonging to concepts in $M_i$, and $\hat y_i$ is the model output (assumed to be a scalar) while removing concepts masked by $M_i$. We repeat this process $K$ times and, similar to RISE~\cite{petsiuk2018rise}, calculate the final concept importance scores, $\textbf{S} \in \mathbb{R}^Q$, through a weighted sum of the performances and the set of masks, as

\begin{equation}
    \textbf{S} = \sum_i^K \hat y_i  M_i.
\end{equation}


% One might be inclined to apply the traditional `occlusion' method~\cite{fel2023holistic} and calculate the importance by recording the performance drop after setting all tokens that belong to a certain concept to zero. However, complex video tasks, \eg object tracking, admit degenerate performance (and thus important scores) if any crucial tokens early in the video are removed. Therefore, we propose \textit{soft concept occlusions} and quantify concept importance based on occluding concepts via the CNMF assignment matrix, $\textbf{G}$. More specifically, for all tubelets belonging to a single video, $\textbf{T}_l[:,j:k]$, the matrix $\textbf{G}[j:k,i]$ indicates precisely how much each tubelet from the video belongs to a given concept, $\textbf{C}^i$. We then occlude a concept via the equation:

\begin{figure}
    \centering   
\includegraphics[width=0.49\textwidth]{figures/methods/CRISv1.pdf}
    \caption{A visual representation of Concept Randomized Importance Sampling (CRIS). Given a video, we generate $K$ models, \{$f_{\textbf{M}_1},...,f_{\textbf{M}_K}\}$, each with a unique mask applied to a given unit of interest (\eg concepts, attention heads). Then, we take a weighted average of the masks according to the performance of the model with the masking applied, to get a final importance ranking of the unit.}
    \label{fig:CRIS_Method}
\end{figure}

\subsection{Discovering Rosetta concepts}\label{sec:Rosetta}
In addition to revealing what spatiotemporal mechanisms exist in individual models with \AlgName, we now describe our method to validate the hypothesis that there exist \textit{universal} mechanisms for learning spatiotemporal representations across architectures and tasks. Formally, we apply \AlgName using the same videos with a set of $R$ models, $\{f^1,...,f^R\}$, resulting in discovered concepts for model, $\textbf{C}^r = \{c^r_1, ..., c^r_i\}$, and corresponding importance scores for each concept, $\textbf{S}^r = \{s^r_1, ..., s^r_i\}$. We aim to measure the similarity between all concept $r$-tuples between the models. More specifically, given the binary support masks for all analyzed videos, $B^r_i$, we compare the similarity via the intersection-over-union (IoU) metric to produce the Rosetta score, $R_{IoU}$, of a concept set, as
\begin{equation}
    R_{IoU} = \frac{|B^{1}_i \cap ... \cap B^{r}_j|}{|B^{1}_i \cup ... \cup B^{r}_j|}.
\end{equation}
Before computing $R_{IoU}$, we filter by concept importance scores, $\{S^1,...,S^r\}$, and only consider the most important $p\%$ of  concepts for each model. This simultaneously produces Rosetta concepts that are more meaningful to all models and exponentially reduces the number of comparisons.

==> sec/5_application.tex <==
\begin{table}[t]
    \centering
    %\resizebox{0.4\textwidth}{!}{
    \begin{tabular}{lll}
        \toprule
         Model & Accuracy $\uparrow$ & GFLOPs $\downarrow$ \\
         \midrule
         % \Xhline{3\arrayrulewidth}
         Baseline & 37.1 & 180.5 \\
         \midrule % hline
         VTCD 33\% Pruned & \textbf{41.4} & 121.5 \\
         VTCD 50\% Pruned & 37.8 & \textbf{91.1} \\
         \bottomrule
    \end{tabular}
    \vspace{-0.25cm}
    \caption{Pruning unimportant heads in VideoMAE results in improved efficiency and accuracy when targeting a subset of classes. Here, we target the six SSv2 classes containing types of spills.}
    \vspace{-0.5cm}
    \label{tab:ApplicationResults}
\end{table}

\begin{table}[t]
\centering
\resizebox{0.4\textwidth}{!}{
        \begin{tabular}{lccc}
            \hline
            Features  & VTCD  & VTCD + SAM~\cite{kirillov2023segment} \\
            \hline
            VideoMAE-SSL& 45.0  & 63.8 \\
            VideoMAE & 43.1 & 64.1 \\            
            InternVideo & 45.8 & 62.3 \\
            % TCOW & \bf{59.9}  & \bf{76.6} \\
        \end{tabular}}
    \caption{We apply VTCD to discover object tracking concepts and evaluate them with mIoU on the DAVIS'16 Validation set.}
    \label{tab:VOS}
\end{table}

\section{\AlgName Applications}\label{sec:Application} 
\smallsec{Concept pruning with \AlgName. }%\label{sec:ConceptPruning} 
% Motivated by the findings that different self-attention heads focus on class-specific concepts (Section~\ref{sec:Experiments}), a key insight is that if there is ever a scenario where you care about a subset, this provides an addiitional way to gain performance + efficiency without training anything
%Consider a large video transformer model trained for $K$ classes where, at deployment, the user cares only about a subset of classes $K_d \subset K$. 
%Traditionally, the user has two options: (i) use the model as is (where many of the parameters and concepts are used for classes outside $K_d$) or (ii) finetune the model on solely the subset to slightly improve performance. 
Consider a video transformer model trained for $K$ classes, but during deployment, the user is only interested in a subset of classes, $K_d \subset K$. Typically, they can either utilize the model as is, with many parameters dedicated to classes outside $K_d$, or enhance performance by finetuning the model solely on the subset.
Motivated by the findings that different self-attention heads focus on class-specific concepts (Section~\ref{sec:ExpValidation}), we instead propose a simple method leveraging \AlgName to prune unimportant heads to $K_d$ and improve model performance and efficiency without finetuning. 

% CRIS allows us to rank the importance of concepts to a given task (\eg classification). Given this ranking, a natural question to ask is whether unimportant concepts can be pruned. Given that previous work has shown a large number of tokens~\cite{} (ICCV23) or heads~\cite{} (NLP paper) in a transformer without harming performance, we hypothesize that pruning unimportant concepts related to \textit{classes one does not care about} can actually \textit{improve performance}. 



We choose the VideoMAE model trained on the SSv2 dataset and focus on the six classes where a `spill' happens (listed in the supplement).
%, where the user wants to be able to categorize the type of accident occurring (\eg in a restaurant setting). 
% We then use \AlgName to discover and score all the concepts in VideoMAE according to their effect on performance on those six classes using the training set and report the results for pruning the least important of them on the validation set in Table~\ref{tab:ApplicationResults}. 
We then use CRIS to rank all the heads in VideoMAE according to their effect on performance on those six classes using the training set and report the results for pruning the least important of them on the validation set in Table~\ref{tab:ApplicationResults}. 
Pruning the 33\% least important heads actually \textit{improves} the accuracy by 4.3\% while reducing FLOPS from 180.5 to 121.5. Further removing 50\% of the heads retains the full performance of the original model (+0.7\%) and reduces FLOPs to 91.1. These results suggest that one can control the trade-off between performance and computation by choosing the number of heads to remove. 


\smallsec{Zero-Shot Semi-Supervised VOS with \AlgName}%\label{sec:ConceptPruning} 
We now demonstrate how \AlgName can be used to turn any pre-trained video transformer into a video object segmentation (VOS) approach. To this end, we run VTCD on the training set of the DAVIS16 benchmark~\cite{perazzi2016benchmark} and select concepts that have the highest overlap with the ground-truth tracks. 
We choose DAVIS16 over DAVIS17 due to the DAVIS17 benchmark containing several query objects smaller than the feature map resolution of the video transformers used in this study. 
We then use these concepts to track new objects on the validation set and report results in Table~\ref{tab:VOS}. 
While a solid performance is achieved by all representations, segmentation accuracy is limited by the low resolution of the concept masks. 
To mitigate this, we introduce a simple refinement step that samples random points inside the masks to prompt SAM~\cite{kirillov2023segment}. 
The resulting approach, shown as VTCD + SAM, significantly improves performance, with even representations not trained for tracking outperforming some dedicated VOS methods in the literature. We anticipate that future developments in video representation learning will automatically lead to better VOS methods with the help of VTCD.


